Sliding Window Recurrences for Sequence Models

Multi-hybrid architectures are poised to take over language modeling due to better quality and performance. We introduce a hierarchical decomposition framework for linear recurrences that allows us to develop algorithms aligned with GPU memory hierarchies, yielding Sliding Window Recurrences. We focus specifically on truncating recurrences to hardware-aligned windows which are naturally jagged, limiting costly inter-warp communication. Using SWR, we develop Phalanx layers that serve as drop-in replacements for windowed attention or linear recurrences. In 1B parameter multi-hybrid models, Phalanx achieves over 10-40% speedup across 4K to 32K context length over optimized Transformers while matching perplexity.

==> catchy_matrix_values.tex <==

    \expandafter\def\csname valSWA00\endcsname{1.000000}
    \expandafter\def\csname valSWA10\endcsname{0.641331}
    \expandafter\def\csname valSWA11\endcsname{0.352254}
    \expandafter\def\csname valSWA20\endcsname{0.382351}
    \expandafter\def\csname valSWA21\endcsname{0.221751}
    \expandafter\def\csname valSWA22\endcsname{0.383068}
    \expandafter\def\csname valSWA30\endcsname{0.318980}
    \expandafter\def\csname valSWA31\endcsname{0.267091}
    \expandafter\def\csname valSWA32\endcsname{0.319175}
    \expandafter\def\csname valSWA33\endcsname{0.075509}
    \expandafter\def\csname valSWA40\endcsname{0.292445}
    \expandafter\def\csname valSWA41\endcsname{0.212146}
    \expandafter\def\csname valSWA42\endcsname{0.292768}
    \expandafter\def\csname valSWA43\endcsname{0.018503}
    \expandafter\def\csname valSWA44\endcsname{0.158478}
    \expandafter\def\csname valSWA51\endcsname{0.168731}
    \expandafter\def\csname valSWA52\endcsname{0.152473}
    \expandafter\def\csname valSWA53\endcsname{0.337143}
    \expandafter\def\csname valSWA54\endcsname{0.184732}
    \expandafter\def\csname valSWA55\endcsname{0.131261}
    \expandafter\def\csname valSWA62\endcsname{0.282682}
    \expandafter\def\csname valSWA63\endcsname{0.024725}
    \expandafter\def\csname valSWA64\endcsname{0.163051}
    \expandafter\def\csname valSWA65\endcsname{0.430975}
    \expandafter\def\csname valSWA66\endcsname{0.072906}
    \expandafter\def\csname valSWA73\endcsname{0.000000}
    \expandafter\def\csname valSWA74\endcsname{0.083037}
    \expandafter\def\csname valSWA75\endcsname{0.384485}
    \expandafter\def\csname valSWA76\endcsname{0.021051}
    \expandafter\def\csname valSWA77\endcsname{0.485766}
    \expandafter\def\csname valSWA84\endcsname{0.156502}
    \expandafter\def\csname valSWA85\endcsname{0.028846}
    \expandafter\def\csname valSWA86\endcsname{0.548373}
    \expandafter\def\csname valSWA87\endcsname{0.021348}
    \expandafter\def\csname valSWA88\endcsname{0.219271}
    \expandafter\def\csname valSWA95\endcsname{0.209149}
    \expandafter\def\csname valSWA96\endcsname{0.134582}
    \expandafter\def\csname valSWA97\endcsname{0.217236}
    \expandafter\def\csname valSWA98\endcsname{0.155536}
    \expandafter\def\csname valSWA99\endcsname{0.257836}
    \expandafter\def\csname valSWA106\endcsname{0.216044}
    \expandafter\def\csname valSWA107\endcsname{0.187371}
    \expandafter\def\csname valSWA108\endcsname{0.207013}
    \expandafter\def\csname valSWA109\endcsname{0.177940}
    \expandafter\def\csname valSWA1010\endcsname{0.185971}
    \expandafter\def\csname valSWA117\endcsname{0.183706}
    \expandafter\def\csname valSWA118\endcsname{0.018381}
    \expandafter\def\csname valSWA119\endcsname{0.538321}
    \expandafter\def\csname valSWA1110\endcsname{0.215123}
    \expandafter\def\csname valSWA1111\endcsname{0.018809}
    \expandafter\def\csname valSWA128\endcsname{0.114534}
    \expandafter\def\csname valSWA129\endcsname{0.387401}
    \expandafter\def\csname valSWA1210\endcsname{0.272837}
    \expandafter\def\csname valSWA1211\endcsname{0.115327}
    \expandafter\def\csname valSWA1212\endcsname{0.084240}
    \expandafter\def\csname valSWA139\endcsname{0.162493}
    \expandafter\def\csname valSWA1310\endcsname{0.174749}
    \expandafter\def\csname valSWA1311\endcsname{0.208139}
    \expandafter\def\csname valSWA1312\endcsname{0.221424}
    \expandafter\def\csname valSWA1313\endcsname{0.207534}
    \expandafter\def\csname valSWA1410\endcsname{0.588674}
    \expandafter\def\csname valSWA1411\endcsname{0.096447}
    \expandafter\def\csname valSWA1412\endcsname{0.048732}
    \expandafter\def\csname valSWA1413\endcsname{0.099510}
    \expandafter\def\csname valSWA1414\endcsname{0.140976}
    \expandafter\def\csname valSWA1511\endcsname{0.197530}
    \expandafter\def\csname valSWA1512\endcsname{0.243553}
    \expandafter\def\csname valSWA1513\endcsname{0.195586}
    \expandafter\def\csname valSWA1514\endcsname{0.174938}
    \expandafter\def\csname valSWA1515\endcsname{0.162732}

    \expandafter\def\csname valLR00\endcsname{1.000000}
    \expandafter\def\csname valLR10\endcsname{0.975551}
    \expandafter\def\csname valLR11\endcsname{1.000000}
    \expandafter\def\csname valLR20\endcsname{0.889411}
    \expandafter\def\csname valLR21\endcsname{0.911715}
    \expandafter\def\csname valLR22\endcsname{1.000000}
    \expandafter\def\csname valLR30\endcsname{0.776189}
    \expandafter\def\csname valLR31\endcsname{0.795674}
    \expandafter\def\csname valLR32\endcsname{0.872800}
    \expandafter\def\csname valLR33\endcsname{1.000000}
    \expandafter\def\csname valLR40\endcsname{0.576817}
    \expandafter\def\csname valLR41\endcsname{0.591338}
    \expandafter\def\csname valLR42\endcsname{0.648816}
    \expandafter\def\csname valLR43\endcsname{0.743611}
    \expandafter\def\csname valLR44\endcsname{1.000000}
    \expandafter\def\csname valLR50\endcsname{0.428232}
    \expandafter\def\csname valLR51\endcsname{0.439053}
    \expandafter\def\csname valLR52\endcsname{0.481888}
    \expandafter\def\csname valLR53\endcsname{0.552533}
    \expandafter\def\csname valLR54\endcsname{0.743604}
    \expandafter\def\csname valLR55\endcsname{1.000000}
    \expandafter\def\csname valLR60\endcsname{0.305159}
    \expandafter\def\csname valLR61\endcsname{0.312916}
    \expandafter\def\csname valLR62\endcsname{0.343622}
    \expandafter\def\csname valLR63\endcsname{0.394264}
    \expandafter\def\csname valLR64\endcsname{0.531232}
    \expandafter\def\csname valLR65\endcsname{0.715028}
    \expandafter\def\csname valLR66\endcsname{1.000000}
    \expandafter\def\csname valLR70\endcsname{0.289951}
    \expandafter\def\csname valLR71\endcsname{0.297330}
    \expandafter\def\csname valLR72\endcsname{0.326537}
    \expandafter\def\csname valLR73\endcsname{0.374707}
    \expandafter\def\csname valLR74\endcsname{0.504990}
    \expandafter\def\csname valLR75\endcsname{0.679815}
    \expandafter\def\csname valLR76\endcsname{0.950878}
    \expandafter\def\csname valLR77\endcsname{1.000000}
    \expandafter\def\csname valLR80\endcsname{0.252705}
    \expandafter\def\csname valLR81\endcsname{0.259157}
    \expandafter\def\csname valLR82\endcsname{0.284693}
    \expandafter\def\csname valLR83\endcsname{0.326809}
    \expandafter\def\csname valLR84\endcsname{0.440718}
    \expandafter\def\csname valLR85\endcsname{0.593572}
    \expandafter\def\csname valLR86\endcsname{0.830569}
    \expandafter\def\csname valLR87\endcsname{0.873517}
    \expandafter\def\csname valLR88\endcsname{1.000000}
    \expandafter\def\csname valLR90\endcsname{0.228177}
    \expandafter\def\csname valLR91\endcsname{0.234018}
    \expandafter\def\csname valLR92\endcsname{0.257137}
    \expandafter\def\csname valLR93\endcsname{0.295266}
    \expandafter\def\csname valLR94\endcsname{0.398393}
    \expandafter\def\csname valLR95\endcsname{0.536778}
    \expandafter\def\csname valLR96\endcsname{0.751341}
    \expandafter\def\csname valLR97\endcsname{0.790224}
    \expandafter\def\csname valLR98\endcsname{0.904734}
    \expandafter\def\csname valLR99\endcsname{1.000000}
    \expandafter\def\csname valLR100\endcsname{0.159200}
    \expandafter\def\csname valLR101\endcsname{0.163323}
    \expandafter\def\csname valLR102\endcsname{0.179645}
    \expandafter\def\csname valLR103\endcsname{0.206563}
    \expandafter\def\csname valLR104\endcsname{0.279367}
    \expandafter\def\csname valLR105\endcsname{0.377062}
    \expandafter\def\csname valLR106\endcsname{0.528537}
    \expandafter\def\csname valLR107\endcsname{0.555988}
    \expandafter\def\csname valLR108\endcsname{0.636828}
    \expandafter\def\csname valLR109\endcsname{0.704083}
    \expandafter\def\csname valLR1010\endcsname{1.000000}
    \expandafter\def\csname valLR110\endcsname{0.156098}
    \expandafter\def\csname valLR111\endcsname{0.160145}
    \expandafter\def\csname valLR112\endcsname{0.176160}
    \expandafter\def\csname valLR113\endcsname{0.202574}
    \expandafter\def\csname valLR114\endcsname{0.274015}
    \expandafter\def\csname valLR115\endcsname{0.369881}
    \expandafter\def\csname valLR116\endcsname{0.518520}
    \expandafter\def\csname valLR117\endcsname{0.545456}
    \expandafter\def\csname valLR118\endcsname{0.624783}
    \expandafter\def\csname valLR119\endcsname{0.690778}
    \expandafter\def\csname valLR1110\endcsname{0.981154}
    \expandafter\def\csname valLR1111\endcsname{1.000000}
    \expandafter\def\csname valLR120\endcsname{0.146576}
    \expandafter\def\csname valLR121\endcsname{0.150386}
    \expandafter\def\csname valLR122\endcsname{0.165463}
    \expandafter\def\csname valLR123\endcsname{0.190329}
    \expandafter\def\csname valLR124\endcsname{0.257585}
    \expandafter\def\csname valLR125\endcsname{0.347834}
    \expandafter\def\csname valLR126\endcsname{0.487763}
    \expandafter\def\csname valLR127\endcsname{0.513121}
    \expandafter\def\csname valLR128\endcsname{0.587800}
    \expandafter\def\csname valLR129\endcsname{0.649929}
    \expandafter\def\csname valLR1210\endcsname{0.923290}
    \expandafter\def\csname valLR1211\endcsname{0.941032}
    \expandafter\def\csname valLR1212\endcsname{1.000000}
    \expandafter\def\csname valLR130\endcsname{0.110100}
    \expandafter\def\csname valLR131\endcsname{0.113001}
    \expandafter\def\csname valLR132\endcsname{0.124484}
    \expandafter\def\csname valLR133\endcsname{0.143421}
    \expandafter\def\csname valLR134\endcsname{0.194641}
    \expandafter\def\csname valLR135\endcsname{0.263373}
    \expandafter\def\csname valLR136\endcsname{0.369940}
    \expandafter\def\csname valLR137\endcsname{0.389252}
    \expandafter\def\csname valLR138\endcsname{0.446126}
    \expandafter\def\csname valLR139\endcsname{0.493442}
    \expandafter\def\csname valLR1310\endcsname{0.701628}
    \expandafter\def\csname valLR1311\endcsname{0.715140}
    \expandafter\def\csname valLR1312\endcsname{0.760049}
    \expandafter\def\csname valLR1313\endcsname{1.000000}
    \expandafter\def\csname valLR140\endcsname{0.081289}
    \expandafter\def\csname valLR141\endcsname{0.083473}
    \expandafter\def\csname valLR142\endcsname{0.092116}
    \expandafter\def\csname valLR143\endcsname{0.106371}
    \expandafter\def\csname valLR144\endcsname{0.144926}
    \expandafter\def\csname valLR145\endcsname{0.196662}
    \expandafter\def\csname valLR146\endcsname{0.276878}
    \expandafter\def\csname valLR147\endcsname{0.291415}
    \expandafter\def\csname valLR148\endcsname{0.334226}
    \expandafter\def\csname valLR149\endcsname{0.369842}
    \expandafter\def\csname valLR1410\endcsname{0.526550}
    \expandafter\def\csname valLR1411\endcsname{0.536721}
    \expandafter\def\csname valLR1412\endcsname{0.570525}
    \expandafter\def\csname valLR1413\endcsname{0.751143}
    \expandafter\def\csname valLR1414\endcsname{1.000000}
    \expandafter\def\csname valLR150\endcsname{0.059643}
    \expandafter\def\csname valLR151\endcsname{0.061287}
    \expandafter\def\csname valLR152\endcsname{0.067797}
    \expandafter\def\csname valLR153\endcsname{0.078534}
    \expandafter\def\csname valLR154\endcsname{0.107573}
    \expandafter\def\csname valLR155\endcsname{0.146540}
    \expandafter\def\csname valLR156\endcsname{0.206958}
    \expandafter\def\csname valLR157\endcsname{0.217907}
    \expandafter\def\csname valLR158\endcsname{0.250151}
    \expandafter\def\csname valLR159\endcsname{0.276977}
    \expandafter\def\csname valLR1510\endcsname{0.395007}
    \expandafter\def\csname valLR1511\endcsname{0.402668}
    \expandafter\def\csname valLR1512\endcsname{0.428129}
    \expandafter\def\csname valLR1513\endcsname{0.564168}
    \expandafter\def\csname valLR1514\endcsname{0.751604}
    \expandafter\def\csname valLR1515\endcsname{1.000000}

    \expandafter\def\csname valSWR00\endcsname{1.000000}
    \expandafter\def\csname valSWR10\endcsname{0.975551}
    \expandafter\def\csname valSWR11\endcsname{1.000000}
    \expandafter\def\csname valSWR20\endcsname{0.889411}
    \expandafter\def\csname valSWR21\endcsname{0.911715}
    \expandafter\def\csname valSWR22\endcsname{1.000000}
    \expandafter\def\csname valSWR30\endcsname{0.776189}
    \expandafter\def\csname valSWR31\endcsname{0.795674}
    \expandafter\def\csname valSWR32\endcsname{0.872800}
    \expandafter\def\csname valSWR33\endcsname{1.000000}
    \expandafter\def\csname valSWR40\endcsname{0.576817}
    \expandafter\def\csname valSWR41\endcsname{0.591338}
    \expandafter\def\csname valSWR42\endcsname{0.648816}
    \expandafter\def\csname valSWR43\endcsname{0.743611}
    \expandafter\def\csname valSWR44\endcsname{1.000000}
    \expandafter\def\csname valSWR50\endcsname{0.428232}
    \expandafter\def\csname valSWR51\endcsname{0.439053}
    \expandafter\def\csname valSWR52\endcsname{0.481888}
    \expandafter\def\csname valSWR53\endcsname{0.552533}
    \expandafter\def\csname valSWR54\endcsname{0.743604}
    \expandafter\def\csname valSWR55\endcsname{1.000000}
    \expandafter\def\csname valSWR60\endcsname{0.305159}
    \expandafter\def\csname valSWR61\endcsname{0.312916}
    \expandafter\def\csname valSWR62\endcsname{0.343622}
    \expandafter\def\csname valSWR63\endcsname{0.394264}
    \expandafter\def\csname valSWR64\endcsname{0.531232}
    \expandafter\def\csname valSWR65\endcsname{0.715028}
    \expandafter\def\csname valSWR66\endcsname{1.000000}
    \expandafter\def\csname valSWR70\endcsname{0.289951}
    \expandafter\def\csname valSWR71\endcsname{0.297330}
    \expandafter\def\csname valSWR72\endcsname{0.326537}
    \expandafter\def\csname valSWR73\endcsname{0.374707}
    \expandafter\def\csname valSWR74\endcsname{0.504990}
    \expandafter\def\csname valSWR75\endcsname{0.679815}
    \expandafter\def\csname valSWR76\endcsname{0.950878}
    \expandafter\def\csname valSWR77\endcsname{1.000000}
    \expandafter\def\csname valSWR84\endcsname{0.440718}
    \expandafter\def\csname valSWR85\endcsname{0.593572}
    \expandafter\def\csname valSWR86\endcsname{0.830569}
    \expandafter\def\csname valSWR87\endcsname{0.873517}
    \expandafter\def\csname valSWR88\endcsname{1.000000}
    \expandafter\def\csname valSWR94\endcsname{0.398393}
    \expandafter\def\csname valSWR95\endcsname{0.536778}
    \expandafter\def\csname valSWR96\endcsname{0.751341}
    \expandafter\def\csname valSWR97\endcsname{0.790224}
    \expandafter\def\csname valSWR98\endcsname{0.904734}
    \expandafter\def\csname valSWR99\endcsname{1.000000}
    \expandafter\def\csname valSWR104\endcsname{0.279367}
    \expandafter\def\csname valSWR105\endcsname{0.377062}
    \expandafter\def\csname valSWR106\endcsname{0.528537}
    \expandafter\def\csname valSWR107\endcsname{0.555988}
    \expandafter\def\csname valSWR108\endcsname{0.636828}
    \expandafter\def\csname valSWR109\endcsname{0.704083}
    \expandafter\def\csname valSWR1010\endcsname{1.000000}
    \expandafter\def\csname valSWR114\endcsname{0.274015}
    \expandafter\def\csname valSWR115\endcsname{0.369881}
    \expandafter\def\csname valSWR116\endcsname{0.518520}
    \expandafter\def\csname valSWR117\endcsname{0.545456}
    \expandafter\def\csname valSWR118\endcsname{0.624783}
    \expandafter\def\csname valSWR119\endcsname{0.690778}
    \expandafter\def\csname valSWR1110\endcsname{0.981154}
    \expandafter\def\csname valSWR1111\endcsname{1.000000}
    \expandafter\def\csname valSWR128\endcsname{0.587800}
    \expandafter\def\csname valSWR129\endcsname{0.649929}
    \expandafter\def\csname valSWR1210\endcsname{0.923290}
    \expandafter\def\csname valSWR1211\endcsname{0.941032}
    \expandafter\def\csname valSWR1212\endcsname{1.000000}
    \expandafter\def\csname valSWR138\endcsname{0.446126}
    \expandafter\def\csname valSWR139\endcsname{0.493442}
    \expandafter\def\csname valSWR1310\endcsname{0.701628}
    \expandafter\def\csname valSWR1311\endcsname{0.715140}
    \expandafter\def\csname valSWR1312\endcsname{0.760049}
    \expandafter\def\csname valSWR1313\endcsname{1.000000}
    \expandafter\def\csname valSWR148\endcsname{0.334226}
    \expandafter\def\csname valSWR149\endcsname{0.369842}
    \expandafter\def\csname valSWR1410\endcsname{0.526550}
    \expandafter\def\csname valSWR1411\endcsname{0.536721}
    \expandafter\def\csname valSWR1412\endcsname{0.570525}
    \expandafter\def\csname valSWR1413\endcsname{0.751143}
    \expandafter\def\csname valSWR1414\endcsname{1.000000}
    \expandafter\def\csname valSWR158\endcsname{0.250151}
    \expandafter\def\csname valSWR159\endcsname{0.276977}
    \expandafter\def\csname valSWR1510\endcsname{0.395007}
    \expandafter\def\csname valSWR1511\endcsname{0.402668}
    \expandafter\def\csname valSWR1512\endcsname{0.428129}
    \expandafter\def\csname valSWR1513\endcsname{0.564168}
    \expandafter\def\csname valSWR1514\endcsname{0.751604}
    \expandafter\def\csname valSWR1515\endcsname{1.000000}


